Measurement of the cross-section for producing a $W$ boson in association with a single top quark in $pp$ collisions at $\sqrt{s}={13}$ TeV with ATLAS

The inclusive cross-section for the associated production of a $W$ boson and top quark is measured using data from proton-proton collisions at $\sqrt{s}={13}$ TeV. The dataset corresponds to an integrated luminosity of 3.2 fb$^{-1}$, and was collected in 2015 by the ATLAS detector at the Large Hadron Collider at CERN. Events are selected requiring two opposite sign isolated leptons and at least one jet; they are separated into signal and control regions based on their jet multiplicity and the number of jets that are identified as containing $b$ hadrons. The $Wt$ signal is then separated from the $t\bar{t}$ background using boosted decision tree discriminants in two regions. The cross-section is extracted by fitting templates to the data distributions, and is measured to be $94 \pm 10$ (stat.)$^{+28}_{-22}$ (syst.) $\pm 2$ (lumi.) pb. The measurement is in agreement with the Standard Model prediction of $\sigma_{\mathrm{theory}} = 71.7 \pm 1.8\,(\mathrm{scale})\,\pm 3.4\,(\mathrm{PDF})\,\mathrm{pb}$.

==> auxiliary.tex <==
\begin{figure}[htbp]
  \centering
  \includegraphics[width=\textwidth]{beforeFit}
  \caption{%
Pre-fit distributions of the signal and control regions
\texttt{1j1b},
 \texttt{2j1b}, and
 \texttt{2j2b}.
 The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.
 The error bands represent the total uncertainties on the predictions.
}
  \label{fig:beforefit_data}
\end{figure}

\input{auxiliarybdt}

\FloatBarrier

\input{tables/prefit_yields}
\input{tables/prefit_yields_ee}
\input{tables/prefit_yields_em}
\input{tables/prefit_yields_mm}
\FloatBarrier

\begin{figure}[htbp]
  \centering
  \includegraphics[width=.48\textwidth]{13TeV/aux/13TeV__Stack__Allregionee}
  \caption{%
    Expected yields of $ee$ events for signal and backgrounds with their total systematic uncertainty (discussed in \Sect{\ref{sec:fit}}) and the number of observed events in the data are shown in the three fit regions (\texttt{1j1b}, \texttt{2j1b}, and \texttt{2j2b}) and the two additional regions (\texttt{1j0b} and \texttt{2j0b}).
    The signal and backgrounds are normalised to their theoretical predictions, and the error bands represent the total systematic uncertainties which are used in this analysis.
  The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
  \label{fig:regions_ee}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=.48\textwidth]{13TeV/aux/13TeV__Stack__Allregionem}
  \caption{%
    Expected yields of $e\mu$ events for signal and backgrounds with their total systematic uncertainty (discussed in \Sect{\ref{sec:fit}}) and the number of observed events in the data are shown in the three fit regions (\texttt{1j1b}, \texttt{2j1b}, and \texttt{2j2b}) and the two additional regions (\texttt{1j0b} and \texttt{2j0b}).
    The signal and backgrounds are normalised to their theoretical predictions, and the error bands represent the total systematic uncertainties which are used in this analysis.
  The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
  \label{fig:regions_em}
\end{figure}

\begin{figure}[htbp]
  \centering
  \includegraphics[width=.48\textwidth]{13TeV/aux/13TeV__Stack__Allregionmm}
  \caption{%
    Expected yields of $\mu\mu$ events for signal and backgrounds with their total systematic uncertainty (discussed in \Sect{\ref{sec:fit}}) and the number of observed events in the data are shown in the three fit regions (\texttt{1j1b}, \texttt{2j1b}, and \texttt{2j2b}) and the two additional regions (\texttt{1j0b} and \texttt{2j0b}).
    The signal and backgrounds are normalised to their theoretical predictions, and the error bands represent the total systematic uncertainties which are used in this analysis.
  The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
  \label{fig:regions_mm}
\end{figure}


==> auxiliarybdt.tex <==
\begin{figure}
  \centering
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__SumET__1j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__DeltaPt_Lep1Lep2_MET__1j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__pt_sys_Lep1METJet1__1j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__Centrality_Lep1Lep2__1j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__DeltaPt_Lep1_MET__1j1b}
  \caption{\label{fig:bdt_input_stack_1j1b_1}%
  Distributions of the \nth{3} to \nth{7} most powerful BDT input variables in the \texttt{1j1b} region. The signal and background are normalised to their expectation. The first and last bins of each distribution contain overflow events. The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__DeltaR_Lep1Lep2_Jet1Jet2__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__mass_Lep1Jet2__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__DeltaPt_Lep1Lep2_MET__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__DeltaPt_Lep1_Jet1__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__mass_Lep1Jet1__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__pt_Lep1__2j1b}
  \caption{\label{fig:bdt_input_stack_2j1b_1}%
  Distributions of the \nth{3} to \nth{8} most powerful BDT input variables in the \texttt{2j1b} region. The signal and background are normalised to their expectation. The first and last bins of each distribution contain overflow events. The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__pt_sys_sig_Lep1Lep2METJet1__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__DeltaR_Lep1_Jet1__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__pt_sys_Jet2__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__pt_sys_sig_Lep1Lep2METJet1Jet2__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__mass_Lep2Jet1Jet2__2j1b}
  \includegraphics[width=.43\textwidth]{13TeV/aux/13TeV__Stack__mass_Lep2Jet1__2j1b}
  \caption{\label{fig:bdt_input_stack_2j1b_2}%
  Distributions of the \nth{9} to \nth{14} most powerful BDT input variables in the \texttt{2j1b} region. The signal and background are normalised to their expectation. The first and last bins of each distribution contain overflow events. The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Stack__mass_Lep2Jet2__2j1b}
  \caption{\label{fig:bdt_input_stack_2j1b_3}%
  Distributions of the \nth{15} most powerful BDT input variable in the \texttt{2j1b} region. The signal and background are normalised to their expectation. The first and last bins of each distribution contain overflow events. The upper panels give the yields in number of events per bin, while the lower panels give the ratios of the numbers of observed events to the total prediction in each bin.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_sys_Lep1Lep2METJet1__1j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaPt_Lep1Lep2_METJet1__1j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__SumET__1j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaPt_Lep1Lep2_MET__1j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_sys_Lep1METJet1__1j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__Centrality_Lep1Lep2__1j1b}
  \caption{\label{fig:bdt_input_overlay_1j1b_1}%
  Distributions of the \nth{1} to \nth{6} most powerful BDT input variables in the \texttt{1j1b} region. The signal and background are normalised to unity. The first and last bins of each distribution contain overflow events.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Overlay__DeltaPt_Lep1_MET__1j1b}
  \caption{\label{fig:bdt_input_overlay_1j1b_2}%
  Distributions of the \nth{7} most powerful BDT input variable in the \texttt{1j1b} region. The signal and background are normalised to unity. The first and last bins of each distribution contain overflow events.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_sys_Lep1Lep2__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaR_Lep1Lep2_METJet1Jet2__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaR_Lep1Lep2_Jet1Jet2__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__mass_Lep1Jet2__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaPt_Lep1Lep2_MET__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaPt_Lep1_Jet1__2j1b}
  \caption{\label{fig:bdt_input_overlay_2j1b_1}%
  Distributions of the \nth{1} to \nth{6} most powerful BDT input variables in the \texttt{2j1b} region. The signal and background are normalised to unity. The first and last bins of each distribution contain overflow events.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__mass_Lep1Jet1__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_Lep1__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_sys_sig_Lep1Lep2METJet1__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__DeltaR_Lep1_Jet1__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_sys_Jet2__2j1b}
  \includegraphics[width=.44\textwidth]{13TeV/aux/13TeV__Overlay__pt_sys_sig_Lep1Lep2METJet1Jet2__2j1b}
  \caption{\label{fig:bdt_input_overlay_2j1b_2}%
  Distributions of the \nth{7} to \nth{12} most powerful BDT input variables in the \texttt{2j1b} region. The signal and background are normalised to unity. The first and last bins of each distribution contain overflow events.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Overlay__mass_Lep2Jet1Jet2__2j1b}
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Overlay__mass_Lep2Jet1__2j1b}
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Overlay__mass_Lep2Jet2__2j1b}
  \caption{\label{fig:bdt_input_overlay_2j1b_3}%
  Distributions of the \nth{13} to \nth{15} most powerful BDT input variables in the \texttt{2j1b} region. The signal and background are normalised to unity. The first and last bins of each distribution contain overflow events.}
\end{figure}

\begin{figure}
  \centering
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Overlay__response_BDT__1j1b}
  \includegraphics[width=.45\textwidth]{13TeV/aux/13TeV__Overlay__response_BDT__2j1b}
  \caption{\label{fig:bdt_response_overlay}%
  Distributions of the BDT response in the \texttt{1j1b} and \texttt{2j1b} regions. The signal and background are normalised to unit. The first and last bins of each distribution contain overflow events.}
\end{figure}



==> tables/mva_separation_2j2b.tex <==
\begin{tabular}{lr}
	\toprule
	\multicolumn{2}{c}{\texttt{2j2b}} \\
	Variable & \multicolumn{1}{c}{$S$} \\
	         & \multicolumn{1}{c}{[$10^{-4}$]} \\
	\midrule

  $m            (\ell_{1} j_{2})$                                      & 4.2 \\
  $\pTsys       (\ell_{1} \ell_{2} \MET)$                              & 4.1 \\
  $\Delta\pT    (\ell_{1} \ell_{2} ,                 j_{2})$           & 3.8 \\
  $\Delta R     (\ell_{1} \ell_{2} ,                 j_{1} j_{2})$     & 3.3 \\
	$m            (\ell_{1} \MET j_{1} j_{2})$                           & 3.3 \\
	$m            (\ell_{1} j_{1})$                                      & 3.3 \\
	$\pT          (j_2)$                                                 & 2.9 \\
  $\Delta\pT    (\ell_{1},                           j_{1})$           & 2.5 \\
  $\Delta R     (\ell_{1},                           j_{1})$           & 2.5 \\
	$m            (\ell_{2} \MET j_{1})$                                 & 2.4 \\
	$m            (\ell_{2} j_{1})$                                      & 2.4 \\
	$m            (\ell_{2} j_{1} j_{2})$                                & 1.9 \\
	$E/m          (\ell_{2} j_{1} j_{2})$                                & 1.1 \\
  $\Delta R     (\ell_{1},                           \ell_{1})$        & 0.8 \\
  $\Delta\phi   (\ell_{1} \ell_{2} j_{1} j_{2},      \MET)$            & 0.8 \\
  $\Delta R     (\ell_{2},                           j_{1})$           & 0.7 \\

	\bottomrule
\end{tabular}


==> tables/prefit_yields.tex <==
\begin{table}
  \centering
  %\setlength{\tabcolsep}{0.0pc}
  \caption{%
    Expected event yields for an integrated luminosity of \lumi.
    Expectations are normalized to cross-section predictions given in \Sect{\ref{sec:samples}}, and the theoretical uncertainty on the cross-section prediction is considered.
  }
  %%\sisetup{round-mode=figures, round-precision=2,group-separator = {}}
  \sisetup{group-separator = {}}
  {%\small
  \begin{tabular}{l
    S[table-format=4.1]@{$\,\pm\,$}S[table-format=3.1]
    S[table-format=4.1]@{$\,\pm\,$}S[table-format=3.1]
    S[table-format=4.2]@{$\,\pm\,$}S[table-format=4.2]}
  	\toprule
  	                          & \multicolumn{2}{c}{\texttt{1j1b}} & \multicolumn{2}{c}{\texttt{2j1b}} & \multicolumn{2}{c}{\texttt{2j2b}} \\
  	\midrule
  	Observed events           & \multicolumn{1}{S[table-format=4.1]@{$\,\phantom{\pm}\,$}}{4254}    &
                              & \multicolumn{1}{S[table-format=4.1]@{$\,\phantom{\pm}\,$}}{6138}    &
                              & \multicolumn{1}{S[table-format=4.2]@{$\,\phantom{\pm}\,$}}{4912}    &  \\
  	\midrule
  	%unrounded values
%    Expected total events       & 4432.10 & 783.88        & 6350.91 & 810.16        & 4900.57 & 1232.05              \\
%  	\midrule
%    Exp.\ $Wt$ events           & 759.30  & 135.21        & 526.49  & 82.39         & 163.57 & 44.57              \\
%    Exp.\ \ttbar events         & 3550.14 & 672.24        & 5644.45 & 750.03        & 4714.48 & 1202.61              \\
%    Exp.\ \Zjets events         & 74.20   & 37.13         & 118.41  & 59.26         & 7.45 & 7.41              \\
%    Exp.\ fake events           & 24.75   & 24.63         & 36.64   & 36.46         & 14.18 & 14.11              \\
%    Exp.\ diboson events        & 23.72   & 5.95          & 24.92   & 6.25          & 0.91 & 0.23              \\
    Expected total events       & 4430 & 780        & 6350 & 810        & 4900 & 1200              \\
  	\midrule
    %without added xs uncertainty  5.36% wt and  5.74% tt
    %Exp.\ $Wt$ events           & 760  & 140        & 526  & 82         & 164  & 45              \\
    %Exp.\ \ttbar events         & 3550 & 670        & 5640 & 750        & 4700 & 1200              \\
    Exp.\ $Wt$ events           & 760  & 140        & 526  & 87         & 164  & 45              \\
    Exp.\ \ttbar events         & 3550 & 700        & 5640 & 820        & 4700 & 1200              \\
    Exp.\ \Zjets events         & 74   & 37         & 118  & 59         & 7.5  & 7.4              \\
    Exp.\ fake events           & 25   & 25         & 37   & 36         & 14   & 14              \\
    Exp.\ diboson events        & 23.7 & 6.0        & 24.9 & 6.3        & 0.91 & 0.23              \\
  	\bottomrule
  \end{tabular}
}
\label{tab:prefit_yields}
\end{table}


==> tables/prefit_yields_ee.tex <==
\begin{table}
  \centering
  %\setlength{\tabcolsep}{0.0pc}
  \caption{%
    Expected yield of $ee$ events for an integrated luminosity of \lumi.
    Expectations are normalized to cross-section predictions given in \Sect{\ref{sec:samples}}, and the theoretical uncertainty on the cross-section prediction is considered.
  }
  %%\sisetup{round-mode=figures, round-precision=2,group-separator = {}}
  \sisetup{group-separator = {}}
  {%\small
  \begin{tabular}{l
    S[table-format=3.2]@{$\,\pm\,$}S[table-format=3.2]
    S[table-format=3.2]@{$\,\pm\,$}S[table-format=3.2]
    S[table-format=3.2]@{$\,\pm\,$}S[table-format=3.2]}
  	\toprule
  	                          & \multicolumn{2}{c}{\texttt{1j1b}} & \multicolumn{2}{c}{\texttt{2j1b}} & \multicolumn{2}{c}{\texttt{2j2b}} \\
  	\midrule
  	Observed $ee$ events           & \multicolumn{1}{S[table-format=3.2]@{$\,\phantom{\pm}\,$}}{576}    &
                                   & \multicolumn{1}{S[table-format=3.2]@{$\,\phantom{\pm}\,$}}{863}    &
                                   & \multicolumn{1}{S[table-format=3.2]@{$\,\phantom{\pm}\,$}}{677}    &  \\
  	\midrule
  	%unrounded
    %Expected $ee$ events      & 620.69 & 118.65          & 929.37 & 126.39          & 662.68 & 173.04              \\
  	%\midrule
    %Exp.\ $ee$ $Wt$ events          & 99.38 & 16.46          & 75.25 & 14.49          & 23.69 & 7.49              \\
    %Exp.\ $ee$ \ttbar events        & 497.37 & 103.01          & 799.51 & 113.65          & 632.21 & 169.40              \\
    %Exp.\ $ee$ \Zjets events        & 12.65 & 6.34          & 41.89 & 21.01          & 2.91 & 2.90              \\
    %Exp.\ $ee$ fake events          & 7.96 & 7.92          & 9.42 & 9.37          & 3.73 & 3.72              \\
    %Exp.\ $ee$ diboson events       & 3.33 & 0.84          & 3.31 & 0.84          & 0.14 & 0.03              \\
    Expected $ee$ events           & 620 & 120          & 929 & 126        & 660 & 170     \\
  	\midrule
    %without added xs uncertainty  5.36% wt and  5.74% tt
    %Exp.\ $ee$ $Wt$ events         & 99 & 16            & 75 & 14          & 23.7 & 7.5            \\
    %Exp.\ $ee$ \ttbar events       & 500 & 100          & 800 & 114        & 630 & 170     \\
    Exp.\ $ee$ $Wt$ events         & 99 & 16            & 75 & 14          & 23.7 & 7.5            \\
    Exp.\ $ee$ \ttbar events       & 500 & 100          & 800 & 114        & 630 & 170     \\
    Exp.\ $ee$ \Zjets events       & 12.7 & 6.3         & 42 & 21          & 2.9 & 2.9              \\
    Exp.\ $ee$ fake events         & 8.0 & 8.0          & 9.4 & 9.4        & 3.7 & 3.7              \\
    Exp.\ $ee$ diboson events      & 3.33 & 0.84        & 3.31 & 0.84      & 0.14 & 0.03              \\
  	\bottomrule
  \end{tabular}
}
\label{tab:prefit_yields_ee}
\end{table}


==> tables/prefit_yields_em.tex <==
\begin{table}
  \centering
  %\setlength{\tabcolsep}{0.0pc}
  \caption{%
    Expected yield of $e\mu$ events for an integrated luminosity of \lumi.
    Expectations are normalized to cross-section predictions given in \Sect{\ref{sec:samples}}, and the theoretical uncertainty on the cross-section prediction is considered.
  }
  %%\sisetup{round-mode=figures, round-precision=2,group-separator = {}}
  \sisetup{group-separator = {}}
  {%\small
  \begin{tabular}{l
    S[table-format=4.1]@{$\,\pm\,$}S[table-format=3.1]
    S[table-format=4.1]@{$\,\pm\,$}S[table-format=3.1]
    S[table-format=4.2]@{$\,\pm\,$}S[table-format=3.2]}
  	\toprule
  	                          & \multicolumn{2}{c}{\texttt{1j1b}} & \multicolumn{2}{c}{\texttt{2j1b}} & \multicolumn{2}{c}{\texttt{2j2b}} \\
  	\midrule
  	Observed $e\mu$ events  & \multicolumn{1}{S[table-format=4.1]@{$\,\phantom{\pm}\,$}}{2795}    &
                            & \multicolumn{1}{S[table-format=4.1]@{$\,\phantom{\pm}\,$}}{3982}    &
                            & \multicolumn{1}{S[table-format=4.2]@{$\,\phantom{\pm}\,$}}{3297}    &  \\
  	\midrule
    Expected $e\mu$ events       & 2890 & 510     & 4100 & 460       & 3270 & 820     \\
  	\midrule
    Exp.\ $e\mu$ $Wt$ events     & 513 & 89       & 344 & 50         & 107 & 27       \\
    Exp.\ $e\mu$ \ttbar events   & 2330 & 440     & 3710 & 430       & 3160 & 800       \\
    Exp.\ $e\mu$ \Zjets events   & 16.8 & 8.4     & 5.4 & 2.7        & 0.03 & 0.03              \\
    Exp.\ $e\mu$ fake events     & 16 & 16        & 24 & 23          & 9.6 & 9.5              \\ 
    Exp.\ $e\mu$ diboson events  & 15.9 & 4.0     & 16.8 & 4.2       & 0.67 & 0.17              \\
  	\bottomrule
  \end{tabular}
}
\label{tab:prefit_yields_em}
\end{table}


==> tables/prefit_yields_mm.tex <==
\begin{table}
  \centering
  %\setlength{\tabcolsep}{0.0pc}
  \caption{%
    Expected yield of $\mu\mu$ events for an integrated luminosity of \lumi.
    Expectations are normalized to cross-section predictions given in \Sect{\ref{sec:samples}}, and the theoretical uncertainty on the cross-section prediction is considered.
  }
  %%\sisetup{round-mode=figures, round-precision=2,group-separator = {}}
  \sisetup{group-separator = {}}
  {%\small
  \begin{tabular}{l
    S[table-format=4.1]@{$\,\pm\,$}S[table-format=3.1]
    S[table-format=4.1]@{$\,\pm\,$}S[table-format=3.1]
    S[table-format=4.2]@{$\,\pm\,$}S[table-format=3.2]}
  	\toprule
  	                          & \multicolumn{2}{c}{\texttt{1j1b}} & \multicolumn{2}{c}{\texttt{2j1b}} & \multicolumn{2}{c}{\texttt{2j2b}} \\
  	\midrule
  	Observed $\mu\mu$ events  & \multicolumn{1}{S[table-format=4.1]@{$\,\phantom{\pm}\,$}}{883}    &
                              & \multicolumn{1}{S[table-format=4.1]@{$\,\phantom{\pm}\,$}}{1293}    &
                              & \multicolumn{1}{S[table-format=4.2]@{$\,\phantom{\pm}\,$}}{938}    &  \\
  	\midrule
  	%
    Expected $\mu\mu$ events      & 930 & 160     & 1330 & 220       & 960 & 240       \\
  	\midrule
    Exp.\ $\mu\mu$ $Wt$ events    & 147 & 26      & 107 & 17         & 32.9 & 9.6       \\
    Exp.\ $\mu\mu$ \ttbar events  & 730 & 140     & 1140 & 210       & 930 & 230       \\
    Exp.\ $\mu\mu$ \Zjets events  & 55 & 28       & 74 & 37          & 4.5 & 4.5       \\
    Exp.\ $\mu\mu$ fake events    & 1.0 & 1.0     & 3.7 & 3.7        & 0.85 & 0.85       \\
    Exp.\ $\mu\mu$ diboson events & 4.5 & 1.1     & 4.8 & 1.2        & 0.11 & 0.03       \\
  	\bottomrule
  \end{tabular}
}
\label{tab:prefit_yields_mm}
\end{table}

